An iterative clustering algorithm for the Contextual Stochastic Block Model with optimality guarantees

Real-world networks often come with side information that can help to improve the performance of network analysis tasks such as clustering. Despite a large number of empirical and theoretical studies conducted on network clustering methods during the past decade, the added value of side information and the methods used to incorporate it optimally in clustering algorithms are relatively less understood. We propose a new iterative algorithm to cluster networks with side information for nodes (in the form of covariates) and show that our algorithm is optimal under the Contextual Symmetric Stochastic Block Model. Our algorithm can be applied to general Contextual Stochastic Block Models and avoids hyperparameter tuning in contrast to previously proposed methods. We confirm our theoretical results on synthetic data experiments where our algorithm significantly outperforms other methods, and show that it can also be applied to signed graphs. Finally we demonstrate the practical interest of our method on real data.

==> algo.tex <==
\section{How to integrate heterogeneous sources of information?}

%One of the main challenge with CSBM is to integrate the two heterogeneous sources of information in the clustering process. 
The use of side information should intuitively help to recover clusters that are not well separated on each individual source of information. However, it is not well understood how to integrate two heterogeneous sources of information in the clustering process. Previous attempts \citep{Binkiewicz2017CovariateassistedSC,CovReg} proceed by directly aggregating the adjacency matrix and a Gram matrix (or Kernel matrix) formed by the covariates, but a lot of information can be lost in the aggregation process. Moreover it is not clear what is the best linear combination of the two matrices. Here we propose a different approach based on a two step algorithm (see Algorithm \ref{alg:ir-csbm}) that fully exploits all information. In the first step we obtain a rough estimate of the model parameters from the previous estimate of the partition; the initialization methods that can be used are discussed in Section \ref{subsec:init}. Then, in the second step, we iteratively refine  the partition, as further explained in Section \ref{subsec:irstep}. In Section \ref{subsec:csbm_not_well_sep} we illustrate via experiments that Algorithm \ref{alg:ir-csbm} outperforms existing methods for cluster recovery in the setting where the clusters are insufficiently separated on a single source of information.

\begin{algorithm}
\caption{Iterative Refinement with Least Squares}\label{alg:ir-csbm}
\begin{flushleft}
        \textbf{Input:} $A\in \R^{n\times n}$, $X\in \R^{n\times d}$,$K\in \mathbb{N}^*$, $\sigma >0$, $Z^{(0)}\in \lbrace 0,1\rbrace ^{n\times K}$ a membership matrix and $T\geq 1$.
\end{flushleft}
        \begin{algorithmic}[1]
    \For{$0 \leq t \leq T-1$}    
        \State  Given $Z^{(t)}$, estimate the model parameters:  $n_k^{(t)} = |\calC_k^{(t)}|$, $W^{(t)}=Z^{(t)}(D^{(t)})^{-1}$ where $D^{(t)}= \diag (n_k^{(t)})_{k\in [K]}$, $\Pi^{(t)}=W^{(t)^\top}AW^{(t)}$ , and $\mu_k^{(t)} = W_{k:}^{(t) \top} X$, for all $k\leq K$.
        \State  Refine the partition by solving for each $i\in [n]$  \scriptsize \[  z_i^{(t+1)}=\arg\min_k ||(A_{i:}W^{(t)}-\Pi^{(t)}_{k:} ) \sqrt{\Sigma^{(t)}_k}||^2  + \frac{||X_i-\mu_k ^{(t)}||^2}{\sigma^2}\] \normalsize where \[\Sigma^{(t)}_k =
            \begin{cases}
            \diag (\frac{n_{k'}^{(t)}}{\Pi_{kk'}^{(t)}} )_{k'\in [K]}  &\text{(\ircsbm)} \\
            \frac{\min_{k'} n_{k'}^{(t)}}{\max_{k',k''}\Pi^{(t)}_{k'k''}}I_K  &\text{(\sircsbm)}\\
            \frac{n}{K(p^{(t)}-q^{(t)})} \log (\frac{p^{(t)}(1-q^{(t)})}{q^{(t)}(1-p^{(t)})})I_K  &\text{(\ircssbm)}
            \end{cases}
            \]
            with $p^{(t)}= K^{-1}\sum_{k\in [K]} \Pi^{(t)}_{kk}$ and $q^{(t)}=(K^2-K)^{-1}\sum_{k\neq k'\in [K]} \Pi^{(t)}_{kk'}$.
        \State Form the matrices $Z^{(t+1)}$ from $z^{(t+1)}$.
        \EndFor
        \end{algorithmic}
 \textbf{Output:} A partition of the nodes $Z^{(T)}$.
\end{algorithm}

\subsection{The refinement mechanism}
\label{subsec:irstep}
At each step $t$,  Algorithm \ref{alg:ir-csbm} estimates the model parameters given a current estimate of the partition ($W^{(t)}$), then updates the partition by reassigning each node to its closest community. Here, the proximity of a node $i$ to a community $k$ is measured by the distance between its estimated (graph) connectivity profile ($A_{i:}W^{(t)}$) and its covariates ($X_{i}$) to the current estimate of the community parameters ($\Pi^{(t)}_{k:}, \mu_k ^{(t)}$). Instead of using the Maximum A Priori (MAP) estimator as in C-EM algorithms, we use a least-square criterion. In a model-based perspective, this can be interpreted as a Gaussian approximation of the SBM. We will see later in the experiments that this doesn't lead to a loss of accuracy, and is also faster.

Different variants of our algorithm are possible depending on the way the variance of each community is estimated and integrated in the criterion used for the partition refinement. The general method will be referred as \ircsbm, the simplified spherical version is denoted by \sircsbm\, and the version of the algorithm used for CSSBM is denoted by \ircssbm.

\textbf{Computational cost.} In each iteration, the complexity of estimating the parameters is $O(nnz(A)+nd)$ while that of estimating the partition is $O(nK(K+d))$. So the total cost of \ircsbm \, is $O(T(nnz(A)+nK(\max (K,d)))$. In our setting $A$ is sparse, hence $nnz(A)\asymp n\log n$.

\begin{remark}
Algorithm \ref{alg:ir-csbm} can also be used for clustering weighted signed graphs, as shown later in the experiments. Moreover, it is  interesting to note that when there are no covariates, the algorithm can be applied to graphs generated from a general SBM. This is in contrast to the iterative algorithm proposed by \cite{Lu2016StatisticalAC} that can only be applied to assortative SBMs (see appendix).
\end{remark}

\subsection{Initialization}
Different strategies can be adopted for initialization. If we assume that the communities are separated on each source of information and that the signal-to-noise ratio (SNR) is large enough to recover a sufficient proportion in each cluster, we can use a spectral method on one source of information (the graph for example). However, it is in general better to combine both sources of information. While one could use the methods proposed in \cite{CovReg} or \cite{Binkiewicz2017CovariateassistedSC} that also come with some theoretical guarantees, we instead use Algorithm \ref{alg:gmm} to initialize the partition. This algorithm will be referred to as \gmm. In our experiments, we used the package \texttt{clusterR} \citep{clusterr} for estimating the Gaussian mixture with an EM algorithm. This algorithm is fast, provides a sufficiently accurate estimate of the partition, and avoids hyperparameter tuning.

\label{subsec:init}
\begin{algorithm}
\caption{EM on graph embedding and covariates (\gmm)}\label{alg:gmm}
\begin{flushleft}
        \textbf{Input:} The number of communities $K$, the adjacency matrix $A$, covariates $X$.
\end{flushleft}
        \begin{algorithmic}[1]
        \State Compute $U_K \in \R ^{n\times K}$ the matrix formed by the eigenvectors associated with the top-$K$ eigenvalues (in absolute order) of $A$.
        \State Merge the columns of $U_K$ with the columns of $X$ to obtain a matrix $X'$.
        \State Cluster the rows of $X'$ by using an EM algorithm for GMM.
        \end{algorithmic}
 \textbf{Output:} A partition of the nodes $Z^{(0)}$.
\end{algorithm}






==> gao_ext.tex <==
Suppose that $l(z^{(t-1)},z) \leq c\tau^{(t-1)}$. Let $i \in [n]$ such that $z_i=a$ and define \[ \delta^{(t)}= \max (\frac{2cK^{1.5}\tau^{(t-1)}}{n\Delta^2_{min}}, \delta ). \] We can assume that $\delta^{(t)}<1$, indeed, it is true by assumption (the initial estimate of the partition is good enough) and the following argument will show that it is true for each $t$.

Recall that  \[ C_i(a,b):=\langle \epsilon_i, \Tilde{\mu}_a-\Tilde{\mu}_b\rangle+ \lambda \langle E_{i:}W, \Tilde{\Pi}_{a:}-\Tilde{\Pi}_{b:}\rangle . \]
Observe that \begin{align*}
    \indic_{\lbrace z_i^{(t)}=b\rbrace}& \leq \indic_{\lbrace C_i(a,b) \leq \frac{-\Delta^2(a,b)}{2} +F_{ib}^{(t-1)}+G_{ib}^{(t-1)}+H_{ib}^{(t-1)} \rbrace }\\
    &\leq \indic_{\lbrace C_i(a,b) \leq \frac{-(1-\delta^{(t)})\Delta^2(a,b)}{2} \rbrace} + \indic_{\lbrace \frac{\delta^{(t)}}{2}\Delta^2(a,b)\leq F_{ib}^{(t-1)}+G_{ib}^{(t-1)}+H_{ib}^{(t-1)}\rbrace}\\
    &\leq \indic_{\lbrace C_i(a,b) \leq \frac{-(1-\delta^{(t)})\Delta^2(a,b)}{2} \rbrace} + \indic_{\lbrace (\frac{\delta^{(t)}}{2}-\max(\frac{\delta}{4}, \frac{cK^{1.5}\tau^{(t-1)}}{2n\Delta_{min}^2}))\Delta^2(a,b)\leq F_{ib}^{(t-1)}\rbrace} \\
    &\leq \indic_{\lbrace C_i(a,b) \leq \frac{-(1-\delta^{(t)})\Delta^2(a,b)}{2} \rbrace} + \indic_{\lbrace \max(\frac{\delta}{4}, \frac{K^{1.5}\tau^{(t-1)}}{n\Delta_{min}^2})\Delta^2(a,b)\leq F_{ib}^{(t-1)}\rbrace}
    \\
    &\leq \indic_{\lbrace C_i(a,b) \leq \frac{-(1-\delta^{(t)})\Delta^2(a,b)}{2} \rbrace} + \indic_{\lbrace \frac{\delta}{4}\Delta^2(a,b)\leq F_{ib}^{(t-1)}\rbrace}\\
    &\leq  \indic_{\lbrace C_i(a,b) \leq \frac{-(1-\delta^{(t)})\Delta^2(a,b)}{2} \rbrace} +\frac{32(F_{ib}^{(t-1)})^2}{\delta^2\Delta^4(a,b)}
\end{align*}
where the last line follows from Markov inequality.

So we obtain \begin{align*}
    \lt &= \sum_{i\in [n]} \sum_{b\in [K]\backslash \lbrace z_i \rbrace}\Delta^2(z_i,b)\indic_{\lbrace z_i^{(t)}=b\rbrace}\\
    & \leq \sum_{i\in [n]} \sum_{b\in [K]\backslash \lbrace z_i \rbrace}\Delta^2(z_i,b) \indic_{\lbrace \langle \epsilon_i, \Tilde{\mu}_{z_i}-\Tilde{\mu}_b\rangle+ \lambda \langle E_{i:}W, \Tilde{\Pi}_{z_i:}-\Tilde{\Pi}_{b:}\rangle \leq \frac{-(1-\delta^{(t)})\Delta^2(z_i,b)}{2} \rbrace}\\
    & +\sum_{i\in [n]} \sum_{b\in [K]\backslash \lbrace z_i \rbrace}\Delta^2(z_i,b)\indic_{\lbrace z_i^{(t)}=b\rbrace}\frac{32(F_{ib}^{(t-1)})^2}{\delta^2\Delta^4(z_i,b)} \\
    & \leq \xi(\delta^{(t)}) + \sum_{i\in [n]}  \max_{b\in [K]\backslash \lbrace z_i \rbrace}\frac{32(F_{ib}^{(t-1)})^2}{\delta^2\Delta^2(z_i,b)} \\
    &\leq \xi(\delta^{(t)}) + \frac{1}{8}l(z^{(t-1)},z).
\end{align*}
Thus \[ \lt \leq \xi(\delta^{(t)}) +\frac{1}{8}\tau^{(t-1)} \leq \frac{7}{8}\tau^{(t-1)} \] since by assumption \ref{cond:ideal} $\xi(\delta^{(t)}) \leq \frac{3}{4}\tau^{(t-1)} $ for all $t$. Let $\tau^{(t)} = \max(\frac{7}{8}\tau^{(t-1)},\tau )$. We can recursively use the same argument to establish the theorem.


==> gao_ext_old.tex <==
Suppose that $l(z^{(t-1)},z) \leq \tau^{(t-1)}$. Let $i \in [n]$ such that $z_i=a$ and define \[ \delta^{(t)}= \max (\frac{2K\tau^{(t-1)}}{n\Delta^2_{min}}, \delta ). \] We can assume that $\delta^{(t)}<1$ because it is true fort $t=1$ by the assumption on the proximity of $z^{(0)}$ to $z$ and the following induction argument will show that the sequence decrease.  

Observe that \begin{align*}
    \indic_{\lbrace z_i^{(t)}=b\rbrace}& \leq \indic_{\lbrace \langle \epsilon_i, \Tilde{\mu}_a-\Tilde{\mu}_b\rangle+ \lambda \langle E_{i:}W, \Tilde{\Pi}_{a:}-\Tilde{\Pi}_{b:}\rangle \leq \frac{-\Delta^2(a,b)}{2} +F_{ib}^{(t-1)}+G_{ib}^{(t-1)}+H_{ib}^{(t-1)} \rbrace }\\
    &\leq \indic_{\lbrace \langle \epsilon_i, \Tilde{\mu}_a-\Tilde{\mu}_b\rangle+ \lambda \langle E_{i:}W, \Tilde{\Pi}_{a:}-\Tilde{\Pi}_{b:}\rangle \leq \frac{-(1-\delta^{(t)})\Delta^2(a,b)}{2} \rbrace} + \indic_{\lbrace \frac{\delta^{(t)}}{2}\Delta^2(a,b)\leq F_{ib}^{(t-1)}+G_{ib}^{(t-1)}+H_{ib}^{(t-1)}\rbrace}\\
    &\leq \indic_{\lbrace \langle \epsilon_i, \Tilde{\mu}_a-\Tilde{\mu}_b\rangle+ \lambda \langle E_{i:}W, \Tilde{\Pi}_{a:}-\Tilde{\Pi}_{b:}\rangle \leq \frac{-(1-\delta^{(t)})\Delta^2(a,b)}{2} \rbrace} + \indic_{\lbrace (\frac{\delta^{(t)}}{2}-\max(\frac{\delta}{4}, \frac{K\tau^{(t-1)}}{2n\Delta_{min}^2}))\Delta^2(a,b)\leq F_{ib}^{(t-1)}+G_{ib}^{(t-1)}\rbrace} \\
    &\leq \indic_{\lbrace \langle \epsilon_i, \Tilde{\mu}_a-\Tilde{\mu}_b\rangle+ \lambda \langle E_{i:}W, \Tilde{\Pi}_{a:}-\Tilde{\Pi}_{b:}\rangle \leq \frac{-(1-\delta^{(t)})\Delta^2(a,b)}{2} \rbrace} + \indic_{\lbrace \max(\frac{\delta}{4}, \frac{K\tau^{(t-1)}}{n\Delta_{min}^2})\Delta^2(a,b)\leq F_{ib}^{(t-1)}+G_{ib}^{(t-1)}\rbrace}
    \\
    &\leq \indic_{\lbrace \langle \epsilon_i, \Tilde{\mu}_a-\Tilde{\mu}_b\rangle+ \lambda \langle E_{i:}W, \Tilde{\Pi}_{a:}-\Tilde{\Pi}_{b:}\rangle \leq \frac{-(1-\delta^{(t)})\Delta^2(a,b)}{2} \rbrace} + \indic_{\lbrace \frac{\delta}{4}\Delta^2(a,b)\leq F_{ib}^{(t-1)}+G_{ib}^{(t-1)}\rbrace}\\
    &\leq  \indic_{\lbrace \langle \epsilon_i, \Tilde{\mu}_a-\Tilde{\mu}_b\rangle+ \lambda \langle E_{i:}W, \Tilde{\Pi}_{a:}-\Tilde{\Pi}_{b:}\rangle \leq \frac{-(1-\delta^{(t)})\Delta^2(a,b)}{2} \rbrace} +\frac{32(F_{ib}^{(t-1)})^2}{\delta^2\Delta^4(a,b)}+\frac{32(G_{ib}^{(t-1)})^2}{\delta^2\Delta^4(a,b)}
\end{align*}
where the last line follows from Markov inequality.

So we obtain \begin{align*}
    \lt &= \sum_{i\in [n]} \sum_{b\in [K]\backslash \lbrace z_i \rbrace}\Delta^2(z_i,b)\indic_{\lbrace z_i^{(t)}=b\rbrace}\\
    & \leq \sum_{i\in [n]} \sum_{b\in [K]\backslash \lbrace z_i \rbrace}\Delta^2(z_i,b) \indic_{\lbrace \langle \epsilon_i, \Tilde{\mu}_{z_i}-\Tilde{\mu}_b\rangle+ \lambda \langle E_{i:}W, \Tilde{\Pi}_{z_i:}-\Tilde{\Pi}_{b:}\rangle \leq \frac{-(1-\delta^{(t)})\Delta^2(z_i,b)}{2} \rbrace}\\
    & +\sum_{i\in [n]} \sum_{b\in [K]\backslash \lbrace z_i \rbrace}\Delta^2(z_i,b)\indic_{\lbrace z_i^{(t)}=b\rbrace}\frac{32(F_{ib}^{(t-1)})^2}{\delta^2\Delta^4(z_i,b)} +\sum_{i\in [n]} \sum_{b\in [K]\backslash \lbrace z_i \rbrace}\Delta^2(z_i,b)\indic_{\lbrace z_i^{(t)}=b\rbrace}\frac{32(G_{ib}^{(t-1)})^2}{\delta^2\Delta^4(z_i,b)}\\
    & \leq \xi(\delta^{(t)}) + \sum_{i\in [n]}  \max_{b\in [K]\backslash \lbrace z_i \rbrace}\frac{32(F_{ib}^{(t-1)})^2}{\delta^2\Delta^2(z_i,b)} + n \max_{i\in [n]}\max_{b\in [K]\backslash \lbrace z_i \rbrace} \frac{32(G_{ib}^{(t-1)})^2}{\delta^2\Delta^2(z_i,b)} \\
    &\leq \xi(\delta^{(t)}) + \frac{1}{8}l(z^{(t-1)},z)+\frac{1}{8}l(z^{(t-1)},z).
\end{align*}
Thus \[ \lt \leq \xi(\delta^{(t)}) +\frac{1}{4}\tau^{(t-1)} \leq \frac{3}{4}\tau^{(t-1)} \] since by assumption \ref{cond:ideal} $\xi(\delta^{(t)}) \leq \frac{1}{4}\tau^{(t-1)} $ for all $t$. Let $\tau^{(t)} = \max(\frac{3}{4}\tau^{(t-1)},\tau )$. We can recursively use the same argument to establish the theorem.


==> preamble.tex <==
%-----------------------------
% Additional packages
%-----------------------------

\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage{amsmath,amssymb,epsfig,amsthm}
\usepackage{graphicx}
\usepackage{comment}
\usepackage{array}
\usepackage{algorithm,algpseudocode}
\usepackage{enumerate}
\usepackage{algpseudocode}
\usepackage{xurl}
\usepackage{xargs}                      % Use more than one optional parameter in a new commands
\usepackage[pdftex,dvipsnames]{xcolor}  % Coloured text etc.
\usepackage[colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}
\usepackage{appendix}
\usepackage[margin=1in]{geometry} 
%\usepackage{hyperref}

\newcommandx{\unsure}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
\newcommandx{\change}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
\newcommandx{\info}[2][1=]{\todo[linecolor=OliveGreen,backgroundcolor=OliveGreen!25,bordercolor=OliveGreen,#1]{#2}}
\newcommandx{\improvement}[2][1=]{\todo[linecolor=Plum,backgroundcolor=Plum!25,bordercolor=Plum,#1]{#2}}
\newcommandx{\thiswillnotshow}[2][1=]{\todo[disable,#1]{#2}}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\allowdisplaybreaks[1]
%\usepackage[round]{natbib}
%\bibliographystyle{unsrtnat}

%-----------------------------
% Theorem like environments
%-----------------------------
\newtheorem{theorem}{Theorem}
\newtheorem{acknowledgment}{Acknowledgment}
\newtheorem{assumption}{Assumption}
\newtheorem{axiom}{Axiom}
\newtheorem{case}{Case}
\newtheorem{claim}{Claim}
\newtheorem{conclusion}{Conclusion}
\newtheorem{condition}{Condition}
\renewcommand{\thecondition}{\Alph{condition}}

\newtheorem{conjecture}{Conjecture}
\newtheorem{corollary}{Corollary}
\newtheorem{criterion}{Criterion}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{exercise}{Exercise}
\newtheorem{lemma}{Lemma}
\newtheorem{notation}{Notation}
\newtheorem{problem}{Problem}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{solution}{Solution}
\newtheorem{summary}{Summary}


\numberwithin{equation}{section}




\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\Hess}{Hess}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\ddiag}{ddiag}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\range}{range}
\DeclareMathOperator{\maximize}{maximize}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Ima}{Im}
\DeclareMathOperator{\maskkpod}{\Omega_U}
%---------------------------------------------
% Commands for symbols used in the report.
% \mathcal symbols
%----------------------------------------------
\newcommand{\calA}{\ensuremath{\mathcal{A}}}
\newcommand{\calB}{\ensuremath{\mathcal{B}}}
\newcommand{\calC}{\ensuremath{\mathcal{C}}}
\newcommand{\calD}{\ensuremath{\mathcal{D}}}
\newcommand{\calH}{\ensuremath{\mathcal{H}}}
\newcommand{\calF}{\ensuremath{\mathcal{F}}}
\newcommand{\calG}{\ensuremath{\mathcal{G}}}
\newcommand{\calI}{\ensuremath{\mathcal{I}}}
\newcommand{\calP}{\ensuremath{\mathcal{P}}}
\newcommand{\calPp}{\ensuremath{\calP^{\prime}}}
\newcommand{\calR}{\ensuremath{\mathcal{R}}}
\newcommand{\calS}{\ensuremath{\mathcal{S}}}
\newcommand{\calM}{\ensuremath{\mathcal{M}}}
\newcommand{\calN}{\ensuremath{\mathcal{N}}}
\newcommand{\calT}{\ensuremath{\mathcal{T}}}
\newcommand{\calU}{\ensuremath{\mathcal{U}}}
\newcommand{\calK}{\ensuremath{\mathcal{K}}}
\newcommand{\calX}{\ensuremath{\mathcal{X}}}
\newcommand{\calV}{\ensuremath{\mathcal{V}}}
\newcommand{\calY}{\ensuremath{\mathcal{Y}}}
\newcommand{\calE}{\ensuremath{\mathcal{E}}}
\newcommand{\calJ}{\ensuremath{\mathcal{J}}}




% Miscellaneous symbols 
\newcommand{\tri}{\ensuremath{\bigtriangleup}}
\newcommand{\norm}[1]{\left\|{#1}\right\|}
\newcommand{\abs}[1]{\left|{#1}\right|}
\newcommand{\ceil}[1]{\lceil{#1}\rceil}
\newcommand{\floor}[1]{\lfloor{#1}\rfloor}
\newcommand{\set}[1]{\left\{{#1}\right\}}
\newcommand{\dotprod}[2]{\langle#1,#2\rangle}
\newcommand{\est}[1]{\widehat{#1}}
\newcommand{\expec}{\ensuremath{\mathbb{E}}}
\newcommand{\matR}{\ensuremath{\mathbb{R}}}
\newcommand{\matZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\argmax}[1]{\underset{#1}{\operatorname{argmax}}}
\newcommand{\argmin}[1]{\underset{#1}{\operatorname{argmin}}}
\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
\newcommand{\prob}{\ensuremath{\mathbb{P}}}
\newcommand{\Linfnorm}{L_{\infty}}

\newcommand{\lt}{l(z^{(t)},z)}

\definecolor{asparagus}{rgb}{0.53, 0.66, 0.42}

\newcommand{\proj}[2]{\mathcal{R}_{#1}(#2)}
\newcommand{\orproj}{\text{Proj}}

% Comments
\newcommand{\hemant}[1]{\textcolor{red}{HT: #1}}
\newcommand{\gb}[1]{\textcolor{cyan}{#1}}
\newcommand{\cb}[1]{\textcolor{purple}{EA: #1}}

%Indicator variable
\newcommand{\indic}{\ensuremath{\mathbf{1}}} 

% Vectors and matrices
\newcommand{\vecx}{\mathbf x}
\newcommand{\vecn}{\mathbf n}
\newcommand{\vecp}{\mathbf p}
\newcommand{\vecq}{\mathbf q}
\newcommand{\veci}{\mathbf i}
\newcommand{\vecj}{\mathbf j}
\newcommand{\vecu}{\mathbf u}
\newcommand{\vecv}{\mathbf v}
\newcommand{\vecw}{\mathbf w}
\newcommand{\vecb}{\mathbf b}
\newcommand{\vecm}{\mathbf m}
\newcommand{\vecc}{\mathbf c}
\newcommand{\vecy}{\mathbf y}
\newcommand{\vecf}{\mathbf f}
\newcommand{\vecz}{\mathbf z}
\newcommand{\veca}{\mathbf a}
\newcommand{\vecg}{\mathbf g}
\newcommand{\veco}{\mathbf 0}
\newcommand{\matA}{\ensuremath{\mathbf{A}}}
\newcommand{\matB}{\ensuremath{\mathbf{B}}}
\newcommand{\matI}{\ensuremath{\mathbf{I}}}
\newcommand{\matV}{\ensuremath{\mathbf{V}}}
\newcommand{\matH}{\ensuremath{\mathbf{H}}}
\newcommand{\matX}{\ensuremath{\mathbf{X}}}
\newcommand{\matP}{\ensuremath{\mathbf{P}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}

%-------------------
% Paper specific 
%
\newcommand{\ircsbm}{\texttt{IR-LS}}
\newcommand{\irmap}{\texttt{IR-MAP}}
\newcommand{\lsc}{\texttt{L-SC}}
\newcommand{\ksc}{\texttt{K-SC}}
\newcommand{\orlsc}{\texttt{ORL-SC}}
\newcommand{\sdp}{\texttt{SDP-Comb}}
\newcommand{\gmm}{\texttt{EM-Emb}}
\newcommand{\asc}{\texttt{A-SC}}
\newcommand{\irmapp}{\texttt{IR-MAP(1)}}
\newcommand{\sircsbm}{\texttt{sIR-LS}}
\newcommand{\irsbm}{\texttt{Iter-SBM}}
\newcommand{\kmeans}{\texttt{K-means}}
\newcommand{\sponge}{\texttt{Sponge}}
\newcommand{\irssbm}{\texttt{IR-SSBM}}
\newcommand{\ircssbm}{\texttt{IR-LSS}}
\newcommand{\spongesym}{\texttt{Sponge-sym}}
